MoCoLSK: Modality Conditioned High-Resolution Downscaling for Land Surface Temperature

Land Surface Temperature (LST) is a critical parameter for environmental studies, but directly obtaining high spatial resolution LST data remains challenging due to the spatio-temporal trade-off in satellite remote sensing. Guided LST downscaling has emerged as an alternative solution to overcome these limitations, but current methods often neglect spatial non-stationarity, and there is a lack of an open-source ecosystem for deep learning methods. In this paper, we propose the Modality-Conditional Large Selective Kernel (MoCoLSK) Network, a novel architecture that dynamically fuses multi-modal data through modality-conditioned projections. MoCoLSK achieves a confluence of dynamic receptive field adjustment and multi-modal feature fusion, leading to enhanced LST prediction accuracy. Furthermore, we establish the GrokLST project, a comprehensive open-source ecosystem featuring the GrokLST dataset, a high-resolution benchmark, and the GrokLST toolkit, an open-source PyTorch-based toolkit encapsulating MoCoLSK alongside 40+ state-of-the-art approaches. Extensive experimental results validate MoCoLSK's effectiveness in capturing complex dependencies and subtle variations within multispectral data, outperforming existing methods in LST downscaling. Our code, dataset, and toolkit are available at https://github.com/GrokCV/GrokLST.

==> contents/3-related-work.tex <==
% !TEX root = ../main.tex
% \bibliography{../reference.bib}

\begin{figure*}[h]
    \centering
    \vspace{-1\baselineskip}
    \includegraphics[width=.7\textwidth]{figs/method/1.pdf}
    \caption{A structural comparison of our proposed MoCoLSK module with other representative unimodal and multimodal attention / selective mechanisms. (f) and (g) are our simple improvements to SK and LSK to enable them to be seamlessly applied to multimodal data fusion tasks. M: Multimodal. K: Kernel.}\label{fig:1}
\end{figure*}

\section{Related Work} \label{sec:related}
% ====================================原稿 start，INTRODUCTION第二段第一句话解释过了
% \textbf{Terminology}: 
% Before we proceed, it is necessary to clarify the specific terminology regarding spatial resolution used in this work. 
% Within the field of computer vision (CV), the terms ``\textit{upscale}'' and ``\textit{downscale}'' are respectively associated with the increase and decrease in spatial resolution, concepts that are synonymous with ``\textit{upsample}'' and ``\textit{downsample}''.
% In contrast, in the context of climate and meteorological studies, as well as remote sensing research, \textbf{``downscaling'' typically refers to the process of increasing the resolution from coarser to finer resolution}, transitioning from a less detailed to a more detailed representation. 
% In this work, we employ the term ``downscaling'' consistent with its usage in remote sensing literature, to indicate an increase in spatial resolution.
% ===================================原稿 end

\subsection{Deep Learning for Downscaling}

In recent years, deep learning models have emerged as a powerful tool for downscaling LR meteorological data to HR outputs. These models leverage the ability of deep neural networks to learn complex spatial and temporal patterns from data, enabling them to effectively capture the relationships between LR and HR data.
% Various deep learning architectures, such as convolutional neural networks (CNNs), recurrent neural networks (RNNs), and their combinations, have been employed for this purpose. Some models also incorporate physics-guided auxiliary variables to further improve the downscaling performance.
% \subsubsection{Dynamical Downscaling}

% One notable work in this domain is the Super Resolution Deep Residual Network \cite{WR2021SRDRN}, which effectively downscales daily precipitation and temperature data.
% Several studies have focused on downscaling specific meteorological variables. For example, Mital et al. present a high-resolution (400 m) gridded dataset of daily precipitation and mean temperature for a mountainous region using a downscaling framework that leverages data-driven models to elucidate topographic influences on climate variables \cite{ESSD2022Precipitation}. Vaughan \textit{et al.}\ employ convolutional conditional neural processes to introduce a flexible deep learning framework for multisite statistical downscaling \cite{GDM2022Convolutional}, capable of generating continuous stochastic predictions for temperature and precipitation at any geographical coordinate.

% For the high-resolution climate data generation task, 
% ===========================================原稿 start
In the context of HR climate data generation, the Super Resolution Deep Residual Network stood out for its effective downscaling of daily meteorological elements like precipitation and temperature \cite{WR2021SRDRN}.
Building upon this, Mital \textit{et al.}\ contributed a fine-scale (400 m) dataset, achieved via a data-driven downscaling model that discerned the impact of topography on climate variables \cite{ESSD2022Precipitation}. 
Furthermore, Vaughan \textit{et al.}\ introduced convolutional conditional neural processes, a versatile deep learning framework for multisite statistical downscaling, which enabled the generation of continuous stochastic forecasts for climate variables across any geographic location \cite{GDM2022Convolutional}.
% ===========================================原稿 end


% Other studies have explored the application of deep learning for downscaling remote sensing data. Yu \textit{et al.}\ present a DisTrad-Super-Resolution Convolutional Neural Network downscaling model that synergizes statistical algorithms with deep learning to enhance the spatial and temporal resolution of remote sensing images \cite{JSTARS2021TemperatureDownscaling}, providing a more accurate analysis of lake surface water temperature dynamics. 
% Mukherjee and Liu introduce a deep learning-based approach that employs an encoder-decoder superresolution architecture with a custom loss function and self-attention mechanism to effectively downscale MODIS spectral bands to a finer resolution \cite{mukherjee2021downscaling}, preserving spatial and spectral integrity without the need for additional spatial information.

% ===========================================原稿 start
Shifting focus to remote sensing data enhancement, Yu \textit{et al.}\ introduced a DisTrad-Super-Resolution Convolutional Network, integrating statistical methods with deep learning to significantly improve the spatial and temporal resolutions of remote sensing imagery \cite{JSTARS2021TemperatureDownscaling}. This advancement allowed for a more refined analysis of lake surface temperature dynamics.
Complementarily, Mukherjee and Liu developed an encoder-decoder super-resolution architecture that incorporated a custom loss function and a self-attention mechanism, adeptly increasing the resolution of MODIS spectral bands while maintaining spatial and spectral fidelity without supplementary spatial inputs \cite{mukherjee2021downscaling}.
% ===========================================原稿 end


Deep learning has also been applied to bias correction and downscaling of climate model simulations. Ba\~no-Medina \textit{et al.}\ provide a comprehensive evaluation of convolutional neural networks for continental-scale statistical downscaling, leveraging the VALUE framework to compare various CNN complexities against traditional models, and emphasizing their superior performance in precipitation downscaling and their potential in climate change projections due to their robust extrapolation abilities \cite{gmd-13-2109-2020}. Wang and Tian address biases in climate model simulations by leveraging deep learning to preserve intervariable dependences and spatial features \cite{wang2022deep}, thereby offering a systematic improvement over traditional univariate and multivariate bias correction methods.

% ===========================================原稿 start
% Deep learning has also played a pivotal role in advancing the precision of climate model simulations through bias correction and downscaling. 
% Ba\~no-Medina \textit{et al.}\ benchmarked convolutional neural networks for continental-scale downscaling within the VALUE framework, demonstrating their enhanced capability in precipitation downscaling and suitability for climate change projections due to their robust extrapolation abilities \cite{gmd-13-2109-2020}.
% Similarly, Wang and Tian applied deep learning to rectify biases in climate simulations, preserving inter-variable dependencies and spatial characteristics, marking an advancement beyond conventional bias correction methods \cite{wang2022deep}.

% ===========================================原稿 end

% While this work focuses on land surface temperature, a meteorological parameter, our approach differs from the straightforward adaptation of deep learning methods in the aforementioned works in two key aspects:
% ===========================================原稿 start 
While the aforementioned works have made strides in applying deep learning to meteorological data downscaling and enhancement, our approach differs in two key aspects that address the limitations of existing methods:
\begin{enumerate}
    \item \textbf{Dynamic Fusion Architecture:} 
    We identified limitations of existing deep learning approaches, mainly fixed receptive fields and uni-dimensional fusion, and proposed a novel dynamic multi-modal fusion architecture. This architecture adaptively modulates receptive fields through modality-conditioned projections, a clear contribution in the field.
    % We delve into the limitations of existing deep learning approaches, namely fixed receptive fields and uni-dimensional fusion, and propose a dynamic multi-modal fusion architecture that adaptively modulates receptive fields through modality-conditioned projections.
    \item \textbf{Open-Source Ecosystem:}
    Beyond methodological contributions, we also aimed to foster reproducible research by establishing an open-source ecosystem. This ecosystem includes a benchmark dataset and a toolkit with implementations of over 40 state-of-the-art methods, distinguishing our work from previous studies.
    % Moreover, this work aims to foster reproducible research by establishing an open-source ecosystem, including a benchmark dataset and a toolkit with implementations of over 40 state-of-the-art methods.
\end{enumerate}
% ==================================原稿 end
% Dynamical downscaling uses regional climate models that incorporate detailed physical processes, complex topography, and other local features to produce high-resolution climate information from coarse global model outputs. It requires bias correction due to reliance on global model accuracy.

% \subsubsection{Statistical Downscaling}

% Statistical downscaling involves creating empirical relationships between historical or processed data and real-time observational data to generate high-resolution gridded data. It relies on statistical methods rather than physical models.

% 二区 - Generating high-resolution daily soil moisture by using spatial downscaling
% In the realm of surface soil moisture (SM) downscaling, the referenced study advances the field by rigorously evaluating the efficacy of various machine learning algorithms, notably emphasizing the superiority of the Random Forest (RF) approach in capturing the complex interplay of geophysical variables across diverse landscapes, while also underlining the nuanced contributions of land surface characteristics to model performance.

% 二区 - A_Machine_Learning-Based_Geostatistical_Downscaling_Method_for_Coarse-Resolution_Soil_Moisture_Products
% In addressing the challenge of coarse spatial resolution in microwave-derived surface soil moisture (SSM) products, the study introduces the support vector area-to-area regression kriging (SVATARK) model, which innovatively merges support vector regression with area-to-area kriging, to account for nonlinear strata-specific variable relationships and the small sample size issue, thereby offering a more precise downscaling technique for enhanced SSM estimation.

% 三区 - 1 Hybrid modelling of random forests and kriging with
% The study introduces a random-forest-based Kriging downscaling approach, utilizing a suite of spectral and spatial predictors, to enhance the spatial resolution of Landsat 8 thermal imagery, offering improved urban thermal detail compared to traditional methods, though it remains limited by the lack of high-resolution ground truth data for validation.

% \subsubsection{Deep Learning-Based Downscaling}

% This category uses deep learning models such as DeepSD, SRCNN, ConvLSTM, FSRCNN, and DCN U-Net to downscale low-resolution meteorological data to high-resolution outputs. These methods often use convolutional neural networks and recurrent neural networks to incorporate both spatial and temporal data, with some models including additional physics-guided auxiliary variables.

% 一区 Top - 2021
% The study introduces the Super Resolution Deep Residual Network (SRDRN), an advanced deep learning model utilizing residual blocks and batch normalization, coupled with data augmentation to effectively downscale daily precipitation and temperature data, showing remarkable skill in capturing extremes and offering significant improvements over traditional methods through transfer learning.

% 一区 Top - 2022-Earth System Science Data-Downscaled hyper-resolution (400 m) gridded datasets of daily precipitation and temperature (2008–2019) for the East–Taylor subbasin (western United States)
% Mital et al. (2021) present a high-resolution (400 m) gridded dataset of daily precipitation and mean temperature for a mountainous region, achieved through a downscaling framework that leverages data-driven models to elucidate topographic influences on climate variables, enhancing the representation of fine-scale hydrological gradients crucial for regional water security studies.


% 一区 Top - 2022 - Convolutional conditional neural processes for
% Employing convolutional conditional neural processes, the research introduces a flexible deep learning framework for multisite statistical downscaling, capable of generating continuous stochastic predictions for temperature and precipitation at any geographical coordinate, with notable advancements in capturing extreme precipitation events.

% 二区 - Research_on_the_Lake_Surface_Water_Temperature_Downscaling_Based_on_Deep_Learning
% The study presents a novel DisTrad-Super-Resolution Convolutional Neural Network (SRCNN) downscaling model that synergizes statistical algorithms with deep learning to enhance the spatial and temporal resolution of remote sensing images, thereby providing a more accurate analysis of lake surface water temperature dynamics.

% 一区 - 2021 - Downscaling MODIS spectral bands using deep learning
% This study introduces a novel deep learning-based approach that employs an encoder-decoder superresolution architecture with a custom loss function and self-attention mechanism to effectively downscale MODIS spectral bands to a finer resolution, preserving spatial and spectral integrity without the need for additional spatial information, thereby offering a robust alternative to traditional interpolation and statistical modeling techniques.

% 一区 Top - 2020 - Configuration and intercomparison of deep learning neural models
% The paper provides a comprehensive evaluation of convolutional neural networks for continental-scale statistical downscaling, leveraging the VALUE framework to compare various CNN complexities against traditional models, and emphasizing their superior performance in precipitation downscaling and their potential in climate change projections due to their robust extrapolation abilities.

% 二区 - On deep learning-based bias correction and downscaling of multiple climate models simulations
% Employing a Super Resolution Deep Residual Network (SRDRN), the study innovatively addresses biases in climate model simulations by leveraging deep learning to preserve intervariable dependences and spatial features, thereby offering a systematic improvement over traditional univariate and multivariate bias correction methods.

% 二区 - A_Bayesian_Deep_Image_Prior_Downscaling_Approach_for_High-Resolution_Soil_Moisture_Estimation
% The article presents a novel Bayesian deep image prior method that combines a fully convolutional neural network with a forward model to statistically enhance the spatial resolution of soil moisture estimation from satellite data, demonstrating a sophisticated integration of deep learning with remote sensing techniques to improve environmental monitoring.

% 一区 Top - 2021
% The study introduces the Super Resolution Deep Residual Network (SRDRN), an advanced deep learning model utilizing residual blocks and batch normalization, coupled with data augmentation to effectively downscale daily precipitation and temperature data, showing remarkable skill in capturing extremes and offering significant improvements over traditional methods through transfer learning.

% 二区Top - An attention mechanism based convolutional network for satellite
% The study advances precipitation downscaling by proposing an attention-based convolutional network that integrates novel global and multi-factor attention modules with a residual learning framework, enhancing the spatial resolution of GPM IMERG data and incorporating a degradation loss function to ensure network robustness across temporal and spatial variations.

% 二区 Top - Downscaling of soil moisture products using deep learning
% In addressing the challenge of low-resolution soil moisture (SM) data, the study innovatively applies deep learning techniques, including deep belief networks and a spatially aware residual network, to downscale microwave products, demonstrating enhanced landscape-level SM variability resolution with improved spatial detail and temporal fidelity on the Tibetan Plateau.

% 二区 Top - Deep learning-based downscaling of tropospheric nitrogen dioxide using
% This research introduces an innovative approach to air quality assessment by using deep learning to integrate high-resolution satellite measurements from TROPOMI with hourly ground-based AirNOW data, employing an inverse distance weighting with a deep neural network and a deep matrix network to downscale daily nitrogen dioxide levels to an hourly resolution, enhancing spatial and temporal monitoring capabilities.

% \subsection{LST Downscaling Dataset}


\subsection{Guided Image Super-Resolution}
% Different from single image super-resolution~\cite{lim2017enhanced,zhang2018image,li2023feature}, guided image super-resolution~\cite{zhao2022discrete,metzger2023guided,yuan2023recurrent,xiang2022detail,zhou2023memory} aims to restore high-resolution images from low-resolution ones, utilizing the  structural information of guidance images from the same scene. 

Guided image super-resolution aims to restore HR images from LR ones by leveraging structural information from guidance images of the same scene, setting it apart from single image super-resolution~\cite{lim2017enhanced,zhang2018image,li2023feature}. Recent advances in guided image super-resolution~\cite{zhao2022discrete,metzger2023guided,yuan2023recurrent,xiang2022detail,zhou2023memory} can be broadly categorized into two main approaches: cross-modal feature fusion and shared-private feature separation.

Cross-modal feature fusion methods focus on effectively combining information from the target and guidance images. 
For instance, Zhong \textit{et al.}\ \cite{zhong2021high} introduced an attention-based hierarchical multi-modal fusion strategy that selected structurally consistent features. 
Building upon this, Shi \textit{et al.} \cite{shi2022symmetric} proposed a symmetric uncertainty-aware transformation to filter out harmful information from the guidance image, ensuring more reliable feature fusion. 
Furthermore, Wang \textit{et al.} \cite{wang2024sgnet} developed a structure-guided method that propagates high-frequency components from the guidance to the target image in both the frequency and gradient domains, enabling more comprehensive fusion of structural details.

% To achieve cross-modal feature fusion, Zhong et al.~\cite{zhong2021high} propose an attention-based hierarchical multi-modal fusion strategy that selects structurally consistent features. Shi et al.~\cite{shi2022symmetric} employ a symmetric uncertainty-aware transformation to filter out harmful information from the guidance for the target. Wang et al.~\cite{wang2024sgnet} introduce a structure guided method that propagates the high-frequency components from the guidance to the target  in both the frequency and gradient domains.

% Most recently, some methods separate the private and shared features between the target and guidance. For example, Deng et al.~\cite{deng2020deep} utilize convolutional sparse coding to split the shared and private information across different modalities. He  et al.~\cite{he2021towards} separate RGB features into high-frequency and low-frequency components using octave convolution. Besides, Zhu et al.~\cite{zhu2023probability} develop a probabilistic global cross-modal upsampling to learn the cross-modal information of the guidance. Xiang et al.~\cite{xiang2022detail} exploit detail injection fusion network to fully utilize the nonlinear complementary features of both the target and guidance.

On the other hand, shared-private feature separation methods aim to disentangle the common and unique information between the target and guidance images. 
Deng \textit{et al.} \cite{deng2020deep} employed convolutional sparse coding to split the shared and private information across different modalities, facilitating more targeted feature fusion. 
Building on this concept, He \textit{et al.} \cite{he2021towards} separated RGB features into high-frequency and low-frequency components using octave convolution, allowing for more fine-grained information integration. 
Similarly, Zhu \textit{et al.} \cite{zhu2023probability} proposed a probabilistic global cross-modal upsampling approach to learn the cross-modal information of the guidance image, enabling more robust feature fusion. 
Additionally, Xiang \textit{et al.} \cite{xiang2022detail} introduced a detail injection fusion network to fully utilize the nonlinear complementary features of both the target and guidance images, achieving more effective detail restoration.

% To some extent, our LST downscaling task can be viewed as a special case of guided image super-resolution. But, out MoCoLSK differs from aforementioned works in two points:
% Our research introduces a novel approach to LST downscaling, which, while conceptually analogous to guided image super-resolution, distinguishes itself in two fundamental aspects:

% ===========================================原稿 start
Our research, while conceptually aligns with guided image super-resolution, introduces a novel approach to LST downscaling that distinguishes itself in two fundamental aspects:
\begin{enumerate}
    \item \textbf{Dynamic Receptive Field:} 
    Existing guided image super-resolution methods often rely on fixed receptive fields, which may not effectively capture the multi-scale dependencies in LST data.
    Our work highlights the significance of dynamic receptive field adjustment for LST downscaling. To the best of our knowledge, this is the first work to emphasize this factor in the field of guided image super-resolution.
    % Our work identifies the importance of dynamic receptive field adjustment for LST downscaling. To the best of our knowledge, this is the first work to emphasize this prior in the field of guided image super-resolution, opening up a new avenue for exploration and improvement.
    \item \textbf{Dynamic Multi-modal Fusion}:
    Previous studies have primarily employed uni-dimensional operations, such as addition, multiplication, or concatenation, for multi-modal fusion. However, these approaches may not fully capture the complex interactions between different modalities.
    Our MoCoLSK framework surpasses traditional uni-dimensional fusion methods by introducing a sophisticated, adaptive interplay between modalities.
    
    % Our methodology, MoCoLSK, features a sophisticated dynamic multi-modal fusion framework. This transcends the traditional uni-dimensional operations employed in previous studies, such as addition, multiplication, or concatenation, introducing a more intricate interplay between modalities.
\end{enumerate}

% ===========================================原稿 end
\subsection{Selective Mechanism}

Our previous work on Selective Kernel Networks (SKNet) \cite{CVPR2019SKNet} introduced a dynamic selection mechanism for convolutional kernels of varying sizes within the network, enabling the adaptation of receptive fields based on the complexity and scale of input features. Building upon this, we proposed Attentional Feature Fusion (AFF) \cite{WACV2021AFF}, which extended the applicability of selective mechanisms to feature fusion tasks by integrating the concept of multi-scale channel attention. More recently, our work on LSKNet \cite{ICCV2023LSK} adapted the selective kernel philosophy for remote sensing object detection tasks, demonstrating the versatility of selective mechanisms in handling HR imagery and the unique challenges posed by varying object scales and backgrounds.

Inspired by the success of SKNet, ResNeSt \cite{CVPR2022ResNeSt} incorporated the selective kernel concept into its architectural design, introducing split-attention blocks that allowed the network to selectively aggregate feature map groups. Similarly, the Self-Calibrated Network (SCNet) \cite{CVPR2020SCNet} employed branch attention and spatial attention to enrich feature representation and bolster localization capabilities. Our MoCoLSK extends the selective kernel concept of LSK to multimodal fusion domain, as illustrated in Fig. \ref{fig:1}, which highlights its differences from existing methods.

% Selective Kernel Networks (SKNet) \cite{CVPR2019SKNet}, a pioneering neural network architecture, introduced a dynamic selection mechanism for convolutional kernels of varying sizes within the network, enabling the adaptation of receptive fields based on the complexity and scale of input features. 
% This adaptability has proven advantageous in diverse application scenarios, ranging from image classification to object detection, where the granularity of features varies significantly.

% Building upon the foundational ideas of SKNet, the work on Attentional Feature Fusion (AFF) \cite{WACV2021AFF} broadened the applicability of selective mechanisms to feature fusion tasks. By integrating the concept of multi-scale channel attention, this approach improved the representational capacity of models, especially in scenarios requiring the synthesis of features across different layers of a network.
% In the same vein, ResNeSt \cite{CVPR2022ResNeSt} incorporated the selective kernel concept into architectural design, introducing split-attention blocks that allowed the network to selectively aggregate feature map groups, enhancing the model's representativeness and robustness to complex visual patterns.
% The Self-Calibrated Network (SCNet) \cite{CVPR2020SCNet} extended the selective paradigm further by employing branch attention to enrich the feature representation and spatial attention to bolster the model's localization capabilities, demonstrating improvements in tasks requiring fine-grained spatial awareness.
% LSKNet \cite{ICCV2023LSK} adapted the selective kernel philosophy for remote sensing object detection tasks, proving the versatility of selective mechanisms in handling high-resolution imagery and the unique challenges posed by varying object scales and backgrounds in such data.

% Our proposed MoCoLSK-Net extends the selective kernel concept, distinguishing itself from these advancements along two key dimensions:


% ===========================================原稿 start
While these advancements have significantly contributed to the field, our proposed MoCoLSK-Net extends the selective kernel concept in two fundamental aspects, addressing the limitations of existing methods:
\begin{enumerate}
  \item \textbf{Single-modal vs. Cross-modal}:
  Previous works primarily focused on fusing features from different receptive fields within the same modality. In contrast, MoCoLSK-Net aims to fuse features from different modalities, enabling the network to leverage complementary information from multiple sources and enhance the overall representation. 
  % While previous works primarily focus on fusing features from different receptive fields within the same modality, MoCoLSK aims to fuse features from different modalities. 
  % This cross-modal fusion enables the network to leverage complementary information from multiple sources and enhance the overall representation.
  % MoCoLSK transcends single-modality limitations by adeptly fusing features across different sensory modalities, thereby harnessing a more comprehensive understanding of the scene.
  \item \textbf{Fixed vs. Dynamic convolution weights:} 
  Existing approaches relied on static convolutional weights for feature fusion. MoCoLSK-Net, on the other hand, dynamically generates attention fusion weights conditioned on multi-modal auxiliary features. This dynamic weighting capability allows MoCoLSK-Net to allocate fusion weights more effectively, tailoring the feature combination process to the nuanced characteristics of multi-modal data.
  
  % Unlike the static convolutional weights employed in previous approaches, MoCoLSK dynamically generates attention fusion weights conditioned on multi-modal auxiliary features. This dynamic weighting capability allows MoCoLSK to allocate fusion weights more effectively, tailoring the feature combination process to the nuanced characteristics of multi-modal data.
  % In MoCoLSK, the convolutional weights that generate attention fusion weights are dynamically conditioned on multi-modal auxiliary features. In contrast, the previous methods employ fixed, static convolutional weights. The dynamic weight generation in MoCoLSK allows for a more adaptive and effective allocation of fusion weights based on the multi-modal context.
\end{enumerate}
% ===========================================原稿 end
